PDE: Gene Effect Inspired Parameter Dynamic Evolution for Low-light Image Enhancement

Low-light image enhancement (LLIE) is a fundamental task in computational photography, aiming to improve illumination, reduce noise, and enhance image quality. While recent advancements focus on designing increasingly complex neural network models, we observe a peculiar phenomenon: resetting certain parameters to random values unexpectedly improves enhancement performance for some images. Drawing inspiration from biological genes, we term this phenomenon the gene effect. The gene effect limits enhancement performance, as even random parameters can sometimes outperform learned ones, preventing models from fully utilizing their capacity. In this paper, we investigate the reason and propose a solution. Based on our observations, we attribute the gene effect to static parameters, analogous to how fixed genetic configurations become maladaptive when environments change. Inspired by biological evolution, where adaptation to new environments relies on gene mutation and recombination, we propose parameter dynamic evolution (PDE) to adapt to different images and mitigate the gene effect. PDE employs a parameter orthogonal generation technique and the corresponding generated parameters to simulate gene recombination and gene mutation, separately. Experiments validate the effectiveness of our techniques. The code will be released to the public.

==> Figure/fig_com_rwdn.tex <==
\begin{figure*}[t]
	\vspace{-1em}
	\centering
	\renewcommand{\arraystretch}{1.5} % 调整行高
	\setlength{\tabcolsep}{1.5pt}
	\scalebox{0.97}{
		\begin{tabular}[b]{ccc ccc}
%			\includegraphics[width=.16\textwidth]{Figure/sidd/noisy_1_18.PNG} &   
%			\includegraphics[width=.16\textwidth]{Figure/sidd/restormer_1_18.PNG} &  
%			\includegraphics[width=.16\textwidth]{Figure/sidd/shuffleformer_1_18.PNG} &  
%			\includegraphics[width=.16\textwidth]{Figure/sidd/NAFNet_1_18.PNG} &   
%			\includegraphics[width=.16\textwidth]{Figure/sidd/NAFNet_ours_1_18.PNG} &  
%			\includegraphics[width=.16\textwidth]{Figure/sidd/clean_1_18.PNG} 
%			\\
			\includegraphics[width=.16\textwidth]{Figure/sidd/noisy_5_18.PNG} &   
			\includegraphics[width=.16\textwidth]{Figure/sidd/restormer_5_18.PNG} &  
			\includegraphics[width=.16\textwidth]{Figure/sidd/shuffleformer_5_18.PNG} &  
			\includegraphics[width=.16\textwidth]{Figure/sidd/NAFNet_5_18.PNG} &   
			\includegraphics[width=.16\textwidth]{Figure/sidd/NAFNet_ours_5_18.PNG} &  
			\includegraphics[width=.16\textwidth]{Figure/sidd/clean_5_18_d.PNG} 
%			\includegraphics[width=.16\textwidth]{Figure/sidd/clean_5_18.PNG} 
%			\\
%			\includegraphics[width=.16\textwidth]{Figure/sidd/noisy_35_1.PNG} &   
%			\includegraphics[width=.16\textwidth]{Figure/sidd/restormer_35_1.PNG} &  
%			\includegraphics[width=.16\textwidth]{Figure/sidd/shuffleformer_35_1.PNG} &  
%			\includegraphics[width=.16\textwidth]{Figure/sidd/NAFNet_35_1.PNG} &   
%			\includegraphics[width=.16\textwidth]{Figure/sidd/NAFNet_ours_35_1.PNG} &  
%			\includegraphics[width=.16\textwidth]{Figure/sidd/clean_35_1.PNG} 
%			\\
%			\includegraphics[width=.16\textwidth]{Figure/sidd/noisy_35_12.PNG} &   
%			\includegraphics[width=.16\textwidth]{Figure/sidd/restormer_35_12.PNG} &  
%			\includegraphics[width=.16\textwidth]{Figure/sidd/shuffleformer_35_12.PNG} &  
%			\includegraphics[width=.16\textwidth]{Figure/sidd/NAFNet_35_12.PNG} &   
%			\includegraphics[width=.16\textwidth]{Figure/sidd/NAFNet_ours_35_12.PNG} &  
%			\includegraphics[width=.16\textwidth]{Figure/sidd/clean_35_12.PNG}
%			\\
%			\includegraphics[width=.16\textwidth]{Figure/sidd/noisy_35_20.PNG} &   
%			\includegraphics[width=.16\textwidth]{Figure/sidd/restormer_35_20.PNG} &  
%			\includegraphics[width=.16\textwidth]{Figure/sidd/shuffleformer_35_20.PNG} &  
%			\includegraphics[width=.16\textwidth]{Figure/sidd/NAFNet_35_20.PNG} &   
%			\includegraphics[width=.16\textwidth]{Figure/sidd/NAFNet_ours_35_20.PNG} &  
%			\includegraphics[width=.16\textwidth]{Figure/sidd/clean_35_20.PNG}
%			\\
%			\includegraphics[width=.16\textwidth]{Figure/sidd/noisy_35_23.PNG} &   
%			\includegraphics[width=.16\textwidth]{Figure/sidd/restormer_35_23.PNG} &  
%			\includegraphics[width=.16\textwidth]{Figure/sidd/shuffleformer_35_23.PNG} &  
%			\includegraphics[width=.16\textwidth]{Figure/sidd/NAFNet_35_23.PNG} &   
%			\includegraphics[width=.16\textwidth]{Figure/sidd/NAFNet_ours_35_23.PNG} &  
%			\includegraphics[width=.16\textwidth]{Figure/sidd/clean_35_23.PNG}
			\\
			\includegraphics[width=.16\textwidth]{Figure/sidd/noisy_35_31.PNG} &   
			\includegraphics[width=.16\textwidth]{Figure/sidd/restormer_35_31.PNG} &  
			\includegraphics[width=.16\textwidth]{Figure/sidd/shuffleformer_35_31.PNG} &  
			\includegraphics[width=.16\textwidth]{Figure/sidd/NAFNet_35_31.PNG} &   
			\includegraphics[width=.16\textwidth]{Figure/sidd/NAFNet_ours_35_31.PNG} &  
%			\includegraphics[width=.16\textwidth]{Figure/sidd/clean_35_31.PNG} 
		\includegraphics[width=.16\textwidth]{Figure/sidd/clean_35_31_d.PNG} 
		\\
%		\vspace{-0.5em}
%		{Noisy image}
		{Input}
		&{Restormer}
		&{ShuffleFormer}
		&{NAFNet}
		&{\bf{NAFNet+Ours}}
%		&{Clean image}
		&{Reference}
		\\
		
		\end{tabular}
	}
%	\vspace{-0.5em}
	\caption{Visual results on the real-world image denoising. 
%		The images denoised by our method exhibit more details and more accurate colors.
	In the top row, the image denoised by our method exhibits more enhanced details.
	In the bottom row, the image denoised by our method exhibits more accurate colors.
	}
	\label{fig:rwdn}
%	\vspace{-1em}
\end{figure*}




==> Figure/random.tex <==
\begin{figure}[t]
	%	\vspace{-1em}
	\centering
	\renewcommand{\arraystretch}{1} % 调整行高
	\setlength{\tabcolsep}{1.5pt}
	\scalebox{0.97}{
		\small
		\begin{tabular}{c c c c}
			\includegraphics[width=.115\textwidth]{Figure/intro_problem/547_random_23.23.png} &
			\includegraphics[width=.115\textwidth]{Figure/intro_problem/547_random_23.56.png} &
			\includegraphics[width=.115\textwidth]{Figure/intro_problem/547_random_25.56.png} &
			\includegraphics[width=.115\textwidth]{Figure/intro_problem/547_random_25.86.png}
			\\
			23.23 dB &
			23.56 dB &
			25.56 dB &
			25.86 dB 
			PSNR
			\\
			
		\end{tabular}
	}
	\vspace{-1em}
	\caption{
		\textbf{Gene effect under different random seeds}. Different random seeds obtain similar enhancement
	}
	\label{fig:random}
\end{figure}


==> Figure/results_redundancy.tex <==

\begin{figure}[t]
	\centering
	\includegraphics[width=\linewidth]{Figure/parameter.pdf} 
	\scalebox{0.97}{
		\small
		\begin{tabular}[b]{ccc}
		{Input Images} & {{Dynamic Convolutions}} & {\textbf{POG (Ours)}}
	\end{tabular}}
%\vspace{-0.5em}
	\caption{\textbf{Comparison of the generated dynamic parameters.} 
		The dynamic parameters generated by POG for each row and column image exhibit gradual evolution processes, indicating that POG recognizes differences and understands similarities between these images.
		(The input low-light images have been brightened for better visibility.)
	}
	\label{fig:comparison}
	\vspace{-1em}
\end{figure}

==> Table/tab_1_obervation_1.tex <==
\begin{table}[tbp]
	\centering
	\small
	\captionof{table}{
		The first observation is that attention layers exhibit greater model redundancy than feedforward layers in transformer architectures. 
	}
	\vspace{-1em}
	\label{table:observation1}
	\setlength{\tabcolsep}{11pt}
	\scalebox{1}{
		\begin{tabular}{l c c c}
			\toprule
			Reset Parameters & All-layers & Latent-layers &\\
			\midrule
%			Attention & {\color{red} -5.52 dB} & {\color{green} +0.02 dB} \\
%			FeedForward & {\color{red} -6.58 dB} & {\color{green} +0.02 dB} \\ 
Attention & {- 5.52 dB}  & {+ 0.02 dB}&  \\
\midrule
FeedForward & {- 6.58 dB}  & {+ 0.02 dB}& \\
			\bottomrule
	\end{tabular}}
%		\vspace{-1em}
\end{table}

